Quaternion Rhapsody

In this paper I explore the set of quaternion algebras over field. Quaternion algebra E(C,-1,-1) is isomorphic to tensor product of complex field C and quaternion algebra H=E(R,-1,-1). Considered two sets of quaternion functions, which satisfy to equation similar to Cauchy-Riemann equation for a complex function.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов, Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин,
Элементы теории функций и функционального анализа,
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Mappings of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010)
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008)
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:q-alg/1004.3007} (2010)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М. Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fihtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Complex.Number.Russian.tex <==
%auto-ignore

\input{\FilePrefix Complex.Number.Eq}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\Section{Линейная функция комплексного поля}
\else
\section{Линейная функция комплексного поля}
\fi
\label{section: Linear Function of Complex Field}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: complex field over real field}
Рассмотрим поле комплексных чисел $C$ как двумерную алгебру над полем действительных чисел.
Положим
\ShowEq{basis of complex field}
базис алгебры $C$.
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Тогда в этом базисе произведение имеет вид
\ShowEq{product of complex field}
и структурные константы имеют вид
\ShowEq{structural constants of complex field}
\fi%Calculus.Paper
Матрица линейной функции
\[
y^{\gi i}=x^{\gi j}f_{\gi j}^{\gi i}
\]
поля комплексных чисел над полем действительных чисел
удовлетворяет соотношению
\begin{align}
\EqLabel{complex field over real field, 0}
f_{\gi 0}^{\gi 0}&=f_{\gi 1}^{\gi 1}
\\
\EqLabel{complex field over real field, 1}
f_{\gi 0}^{\gi 1}&=-f_{\gi 1}^{\gi 0}
\end{align}
\end{theorem}
\begin{proof}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Равенства
\EqRef{product of complex field} и
\EqRef{structural constants of complex field}
следуют из равенства $i^2=-1$.
Пользуясь равенством
\xEqRef{0812.4763}{linear map over field, division ring, relation}
получаем соотношения
\ShowEq{complex field over real field}
Из равенств
\EqRef{complex field over real field, 0, 0} и
\EqRef{complex field over real field, 0, 1}
следует \EqRef{complex field over real field, 0}.
Из равенств
\EqRef{complex field over real field, 1, 0} и
\EqRef{complex field over real field, 1, 1}
следует \EqRef{complex field over real field, 1}.
\else%Calculus.Paper
Смотри доказательство теоремы
\xRef{8433-5163}{theorem: complex field over real field}.
\fi%Calculus.Paper
\end{proof}

\ePrints{0701.238,1003.1544,8433-5163}
\ifx\Semafor\ValueOff
\begin{theorem}[Уравнения Коши\Hyph Римана]
Если матрица
\ShowEq{Jacobian of map of complex variable}
является матрицей Якоби функции комплексного переменного
\[
x=x^{\gi 0}+x^{\gi 1}i\rightarrow y=y^{\gi 0}(x^{\gi 0},x^{\gi 1})+y^{\gi 1}(x^{\gi 0},x^{\gi 1})i
\]
над полем действительных чисел,
то
\ShowEq{Cauchy Riemann equations, complex field, 1}
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: complex field over real field}.
\end{proof}

\begin{theorem}
Производная функции комплексного переменного удовлетворяет равенству
\ShowEq{Cauchy Riemann equations, complex field, 2}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{Cauchy Riemann equations, complex field, 2, 1}
следует из равенств
\EqRef{Cauchy Riemann equations, complex field, 1}.
\end{proof}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
Равенство \EqRef{Cauchy Riemann equations, complex field, 2}
эквивалентно равенству
\ShowEq{Cauchy Riemann equations, complex field, 3}
\fi
\ifx\texFuture\Defined
Производная Гато функции комплексного переменного является
полным дифференциалом и имеет вид
\ShowEq{Gateaux derivative, complex field}
где $dx$, $dy\in R$.
Поэтому символическое уравнение
\ShowEq{Cauchy Riemann equations, Gateaux derivative, complex field}
не выражает связь производной Гато с уравнения Коши\Hyph Римана.
\fi
\fi

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOn
\Section{Алгебра кватернионов}
\else
\section{Алгебра кватернионов}
\fi

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
В этой статье я рассматриваю множество кватернионных алгебр,
определённых в \citeBib{Izrail M. Gelfand: Quaternion Groups}.

\begin{definition}
Пусть $F$ - поле.
Расширение $F(i,j,k)$ поля $F$ называется
\AddIndex{алгеброй
\symb{E(F,a,b)}1{quaternion algebra over the field}
кватернионов над полем $F$}{quaternion algebra over the field}\footnote{Я
буду следовать определению из \citeBib{Izrail M. Gelfand: Quaternion Groups}.},
если произведение в алгебре $E$ определено согласно правилам
\ShowEq{product in E(F,a,b), table}
где $a$, $b\in F$, $ab\ne 0$.
\qed
\end{definition}

Элементы алгебры $E(F,a,b)$ имеют вид
\[
x=x^{\gi 0}+x^{\gi 1}i+x^{\gi 2}j+x^{\gi 3}k
\]
где $x^{\gi i}\in F$, $\gi i=\gi 0$, $\gi 1$, $\gi 2$, $\gi 3$.
Кватернион
\[
\overline x=x^{\gi 0}-x^{\gi 1}i-x^{\gi 2}j-x^{\gi 3}k
\]
называется сопряжённым кватерниону $x$.
Мы определим
\AddIndex{норму кватерниона}{norm of quaternion}
$x$ равенством
\ShowEq{norm of quaternion E(F,a,b)}
Из равенства \EqRef{norm of quaternion E(F,a,b)} следует, что
$E(F,a,b)$ является алгеброй с делением только когда $a<0$, $b<0$.
Тогда мы можем пронормировать базис так, что $a=-1$, $b=-1$.

Мы будем обозначать символом
\ShowEq{quaternion division algebra over the field}
алгебру $E(F,-1,-1)$
кватернионов с делением над полем $F$.
\symb{H}0{quaternion algebra over real field}
Мы будем полагать $\ShowSymbol{quaternion algebra over real field}=E(R,-1,-1)$.
\def\EF{E(F)}
\else
\def\EF{H}
\fi
Произведение в алгебре кватернионов $\EF$ определено согласно правилам
\begin{equation}
\begin{array}{c|ccc}
&i&j&k\\
\hline
i&-1&k&-j\\
j&-k&-1&i\\
k&j&-i&-1\\
\end{array}
\EqLabel{product of quaternions}
\end{equation}
В алгебре $\EF$ норма кватерниона имеет вид
\begin{equation}
\EqLabel{norm of quaternion}
|x|^2=x\overline x=(x^{\gi 0})^2+(x^{\gi 1})^2+(x^{\gi 2})^2+(x^{\gi 3})^2
\end{equation}
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
При этом обратный элемент имеет вид
\begin{equation}
\EqLabel{inverce quaternion}
x^{-1}=|x|^{-2}\overline x
\end{equation}

Внутренний автоморфизм алгебры кватернионов $H$\footnote{См.
\citeBib{Hamilton papers 3}, с. 643.}
\ShowEq{Quaternion Rotation}
описывает вращение вектора с координатами $x$, $y$, $z$.
Если $q$ записан в виде суммы скаляра и вектора
\ShowEq{Quaternion Rotation, 1}
то \EqRef{Quaternion Rotation} описывает вращение
вектора $(x,y,z)$ вокруг вектора $(a,b,c)$ на угол $2\alpha$.
\fi


==> Convention.Russian.tex <==
%auto-ignore
\input{\FilePrefix Convention.Eq}

\section{Соглашения}

\begin{enumerate}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315,1003.1544}
\Items{1006.2597}
\ifx\Semafor\ValueOn
\item Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции,
хотя встречается текст, в котором неясно, какому термину надо
отдать предпочтение.
%Однако мы можем рассматривать свободную
%алгебру как векторное пространство над полем.
%Так как нежелательно одно и тоже соответствие называть то функцией, то
%отображением, я буду пользоваться термином линейная функция алгебры.
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1001.4852}
\Items{1003.1544}
\ifx\Semafor\ValueOn
\item
В любом выражении, где появляется индекс, я предполагаю,
что этот индекс может иметь внутреннюю структуру.
Например, при рассмотрении алгебры $A$ координаты $a\in A$
относительно базиса $\Basis e$ пронумерованы индексом $i$.
Это означает, что $a$ является вектором. Однако, если $a$
является матрицей, нам необходимо два индекса, один нумерует
строки, другой - столбцы. В том случае, когда мы уточняем структуру
индекса, мы будем начинать индекс с символа $\cdot$ в соответствующей
позиции.
Например, если я рассматриваю матрицу $a^i_j$ как элемент векторного
пространства, то я могу записать элемент матрицы в виде $a^{\cdot}{}^i_j$.
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1006.2597,1011.3102}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\item
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $s$.
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\item
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
При этом подразумевается, что отображение мультипликативно над
максимально возможным полем. В частности, линейное отображение
тела $D$ мультипликативно над центром $Z(D)$. Это не противоречит
определению линейного отображения поля, так как для поля $F$ справедливо
$Z(F)=F$.
Если поле $F$ отлично
от максимально возможного, то я это явно указываю в тексте.
\fi

\ePrints{0912.4061}
\ifx\Semafor\ValueOn
\item
Для данного поля $F$, если не оговорено противное,
мы будем рассматривать конечномерную $F$\Hyph алгебру.
%без делителей нуля.
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307}
\ifx\Semafor\ValueOn
\item
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
Запись \Ds линейно зависимые векторы можно прочесть
как D\Hyph star\Hyph линейно зависимые векторы либо
как векторы, линейно зависимые слева.
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597}
\ifx\Semafor\ValueOn
\item Пусть $A$ - свободная конечно
мерная алгебра.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
Однако в алгебре не принято использовать векторные обозначения.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}

\item Если свободная конечномерная алгебра имеет единицу,
то мы будем отождествлять
вектор базиса $\Vector e_{\gi 0}$ с единицей алгебры.
\fi

\ePrints{0906.0135,0912.3315,8443-0072,1102.5168}
\ifx\Semafor\ValueOn
\item В \citeBib{Cohn: Universal Algebra}
произвольная операция алгебры обозначена буквой $\omega$,
и $\Omega$ - множество операций некоторой универсальной алгебры.
Соответственно, универсальная алгебра с множеством операций
$\Omega$ обозначается $\Omega$\Hyph алгебра.
Аналогичные обозначения мы видим в
\citeBib{Burris Sankappanavar} с той небольшой разницей,
что операция в алгебре обозначена буквой $f$
и $\mathcal F$ - множество операций.
Я выбрал первый вариант обозначений, так как в этом случае
легче видно, где я использую операцию.
\fi

\ePrints{0906.0135,0912.3315,8443-0072}
\ifx\Semafor\ValueOn
\item
Так как число универсальных алгебр в башне представлений переменно,
то мы будем пользоваться векторными обозначениями для башни
представлений. Множество
$(A_1,...,A_n)$ $\Omega_i$\Hyph алгебр $A_i$, $i=1$, ..., $n$
мы будем обозначать $\Vector A$. Множество представлений
$(f_{1,2},...,f_{n-1,n})$ этих алгебр мы будем обозначать $\Vector f$.
Так как разные алгебры имеют разный тип, мы также
будем говорить о множестве $\Vector{\Omega}$\Hyph алгебр.
\ePrints{8443-0072}
\ifx\Semafor\ValueOn
Символом
\else
По отношению к множеству $\Vector A$
мы также будем пользоваться матричными обозначениями, предложенными
в разделе \xRef{0701.238}{section: Concept of Generalized Index}.
Например, символом
\fi
$\Vector A_{[1]}$ мы будем обозначать
множество $\Vector{\Omega}$\Hyph алгебр $(A_2,...,A_n)$.
В соответствующем обозначении $(\VX A,\Vector f)$ башни
представлений подразумевается, что $\Vector f=(f_{2,3},...,f_{n-1,n})$.

\item Так как мы пользуемся векторными обозначениями для элементов
башни представлений, необходимо соглашение о записи операций.
Предполагается, что операции выполняются покомпонентно. Например,
\ShowEq{vector notation in tower of representations}
\fi

\ePrints{8443-0072,0906.0135,NewAffine,1102.5168}
\ifx\Semafor\ValueOn
\item
Пусть $A$ - $\Omega_1$\Hyph алгебра.
Пусть $B$ - $\Omega_2$\Hyph алгебра.
Запись
\ShowEq{A->*B}
означает, что определено представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
\fi

\ePrints{0702.561,0707.2246,0803.2620}%,8443-0072}
\ifx\Semafor\ValueOn
\item
Я пользуюсь стрелкой $\xymatrix{\arp[r]&}$
на диаграмме для обозначения проекции расслоения.
\item
Я пользуюсь стрелкой $\xymatrix{\ars[r]&}$
на диаграмме для обозначения сечения расслоения.
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\item
Я считаю диаграммы отображений важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я рассказывал своим коллегам
какие преимущества имеет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.
\fi

\ePrints{1001.4852,1003.1544,1006.2597,1011.3102}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\item Если в некотором выражении используется несколько
операций, среди которых есть операция $\circ$, то предполагается,
что операция $\circ$ выполняется первой.
Ниже приведен пример эквивалентных выражений.
\ShowEq{list circ expressions}
\fi

%\ePrints{0906.0135,NewAffine}
%\ifx\Semafor\ValueOn
%\item
%Пусть $\VX X$ - базис башни представлений $(\Vector A,\Vector f)$.
%Мы будем называть $\Omega_n$\Hyph слово
%$w_n(\Vector f,\VX X,x_n)$ координатами $x_n\in A_n$
%относительно базиса $\VX X$.
%\fi

\ifx\PrintPaper\undefined
\item
Без сомнения, у читателя могут быть вопросы,
замечания, возражения. Я буду признателен любому отзыву.
\fi

\end{enumerate}



==> Epilogue.0909.0855.Russian.tex <==
%auto-ignore

\input{Epilogue.0909.0855.Eq}

\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
\section{Вместо эпилога}

Поле комплексных чисел и алгебра кватернионов имеют и
общие свойства, и некоторые различия.
Эти различия делают более трудной задачу
найти в алгебре кватернионов закономерности,
подобные знакомым нам в поле комплексных чисел.
Поэтому понимание этих различий очень важно.

Одно из направлений исследования - это найти
аналог уравнения Коши\Hyph Римана
в алгебре кватернионов.
В статье я проанализировал некоторые исследования в этой области.
\ifx\texFuture\Defined
При этом я хотел найти связь этих исследований с производной Гато.
Очевидно, что непосредственная попытка решить эту задачу,
опираясь на равенство
\xEqRef{0812.4763}{linear map over field, division ring, relation},
приводит к неудаче.
Следовательно, искомое множество отображений меньше,
чем множество дифференцируемых отображений. 

Я обратил внимание, на сходство равенств
\EqRef{Cauchy Riemann equations, Gateaux derivative, complex field}
и
\EqRef{Cauchy Riemann equations, Gateaux derivative, Regular quaternion function}.
Но мне нужно ещё время, чтобы понять к каким результатам может
привести эта связь.

%Какое-то время эти равенства были для меня загадкой.
%Однако в процессе работы над книгой
%\citeBib{0906.0135}
%я заметил, что если в $D$\Hyph аффинном пространстве определено отображение
%\[
%f:D^n\rightarrow D
%\]
%то условие
%\[
%\partial f(\Vector x)(\Vector a)=0
%\]
%эквивалентно утверждению, что вектор $\Vector a$
%касается поверхности $f(\Vector x)=\const$.
%Этим равенствам можно дать следующую интерпретацию.
%Рассмотрим отображение
%\[
%f:D\rightarrow D
%\]
%Пусть множество точек
%\[
%A=\{x:f(x)=a\}
%\]
%содержит непустое открытое множество $U$.
\fi
\fi

Согласно теореме
\ePrints{Calculus.Paper}
\ifx\Semafor\ValueOff
\xRef{0812.4763}{theorem: complex field over real field}
\else
\ref{theorem: complex field over real field}
\fi
линейное отображение имеет матрицу
\ShowEq{complex linear map, matrix}
Это отображение соответствует умножению на число
\ShowEq{complex linear map, matrix 0}
Утверждение следует из равенств
\ShowEq{complex linear map, matrix 1}

Я решил рассмотреть аналогичный класс функций кватернионов.
Линейное отображение алгебры кватернионов
\ShowEq{linear mapping of quaternion algebra}
имеет матрицу
\ShowEq{linear mapping of quaternion algebra, matrix}

Интересно рассмотреть класс функций кватерниона,
которые имеют производную похожей структуры.
Однако структура матрицы
\EqRef{linear mapping of quaternion algebra, matrix}
мне представляется несколько жёсткой для производной
функции кватернионов и я несколько ослаблю требование.
Я буду предполагать, что производная удовлетворяет
следующим равенствам
\ShowEq{quaternion derivative, request}
Нетрудно убедиться, что производная функции вида
\ShowEq{quaternion function, 1}
удовлетворяет равенствам
\eqref{equation: quaternion derivative, request, 1},
\eqref{equation: quaternion derivative, request, 2}.

Рассмотрим функцию
\ShowEq{quaternion function, 2}
Непосредственное вычисление даёт
\ShowEq{quaternion function, 3}
Производная отображения \EqRef{quaternion function, 3}
имеет матрицу
\ShowEq{quaternion function, 4}
Следовательно, матрица \EqRef{quaternion function, 4}
удовлетворяет равенствам
\eqref{equation: quaternion derivative, request, 1},
\eqref{equation: quaternion derivative, request, 2}.

\begin{theorem}
Производная сопряжения не
удовлетворяет равенствам
\eqref{equation: quaternion derivative, request, 1},
\eqref{equation: quaternion derivative, request, 2}.
\end{theorem}
\begin{proof}
Согласно доказательству теоремы
\xRef{0812.4763}{theorem: quaternion conjugation},
производная сопряжения не
удовлетворяет равенству
\eqref{equation: quaternion derivative, request, 1}.
\end{proof}

Однако множество функций, производная которых
удовлетворяет равенствам
\eqref{equation: quaternion derivative, request, 1},
\eqref{equation: quaternion derivative, request, 2}
не достаточно велико.

\begin{theorem}
Отображение
\ShowEq{quaternion function, y=x3}
не удовлетворяет равенству
\eqref{equation: quaternion derivative, request, 1}.
\end{theorem}
\begin{proof}
Мы можем отображение
\EqRef{quaternion function, y=x3}
представить в виде
\ShowEq{quaternion function, y=xx2}
Координаты этого отображения имеют вид
\ShowEq{quaternion function, 5}
Из равенства
\EqRef{quaternion function, 50},
следует
\ShowEq{quaternion function, 5 00}
Из равенства
\EqRef{quaternion function, 51},
следует
\ShowEq{quaternion function, 5 11}
Утверждение теоремы следует из равенств
\EqRef{quaternion function, 5 00},
\EqRef{quaternion function, 5 11}.
\end{proof}

Без сомнения, это только начало исследования,
и немало вопросов должно быть отвечено.


==> Preface.0909.0855.Russian.tex <==
%auto-ignore

\section{Предисловие}

Когда я начал исследовать математический анализ над телом, я обратил внимание
на большое количество статей, посвящённое регулярным функциям кватернионов и
аналогу уравнения Коши\Hyph Римана. Я хотел понять, появляется ли уравнение Коши\Hyph
Римана в рамках той теории, которую я изучаю. Это и послужило толчком к
рассмотрению тела как векторного пространства над центром.

Введение базиса упрощает некоторые построения и является
своеобразным мостом между производной Гато и матрицей Якоби отображения.
Это именно то место, где должно появиться уравнение Коши\Hyph Римана.
Рассмотрение производной функции комплексных чисел показывает, что уравнение
Коши\Hyph Римана имеет алгебраическую природу и связана с тем,
что существует $R$\Hyph линейная функция поля комплексных
чисел, не являющаяся $C$\Hyph линейной.
Например сопряжение комплексного числа
линейно над полем действительных чисел, но не является
линейным отображением над полем комплексных чисел.

В алгебре кватернионов $H$
существует только $R$\Hyph линейное отображение.
Следствием этого является возможность выразить любое
$R$\Hyph линейное отображение через кватернион
и отсутствие очевидного аналога уравнения Коши\Hyph Римана
в алгебре кватернионов.
Тем не менее, в многочисленных статьях и книгах, посвящённых анализу
над алгеброй кватернионов, математики изучают множества отображений,
свойства которых похожи на свойства функции комплексной переменной.
Некоторые авторы не ограничивают себя алгеброй кватернионов и рассматривают
более общие алгебры.

В статье \citeBib{Izrail M. Gelfand: Quaternion Groups}
Гельфанд рассматривает алгебру кватернионов над произвольным полем и
с произвольными параметрами.
При этом $H=E(R,-1,-1)$.
Опираясь на эту статью, я решил
рассмотреть два случая, которые для меня важны.

Алгебра $E(R,a,b)$ была интересна для меня тем, что я хотел
подобрать параметры $a$, $b$ так, что система линейных уравнений
\xEqRef{0812.4763}{linear map over field, division ring, relation}
становится вырожденной. Мне было важно понять, что произойдёт в этом случае.
При изучении структуры линейного отображения над телом
для меня было не совсем очевидно как повлияет на ответ
вырожденность системы линейных уравнений
\xEqRef{0812.4763}{linear map over field, division ring, relation}.
Однако решение этой задачи не дало ожидаемого ответа.
Система линейных уравнений оказалась настолько простой,
что невооружённым глазом видно, что эта система не может быть вырожденной.

Я писал, что уравнение Коши\Hyph Римана связано с тем,
что поле комплексных чисел имеет подполе действительных чисел. Я высказал
также предположение, что похожее утверждение возможно в алгебрах
с достаточно сложным центром.
Поэтому в алгебре кватернионов над полем комплексных чисел
я ожидал увидеть аналог уравнения
Коши\Hyph Римана.
В ходе решения задачи выяснилось, что алгебра $E(C,-1,-1)$
изоморфна тензорному произведению $C\otimes H$.
Поэтому линейные функции этой алгебры, а следовательно,
и матрица Якоби произвольного
отображения, удовлетворяют уравнению Коши\Hyph Римана для компоненты
тензорного произведения, порождённой полем $C$.
Естественным продолжением этой темы явилось изучение тензорного
произведения $C\otimes(C\otimes H)$. В частности, первое, на что я
обратил внимание, - это неассоциативность тензорного произведения.

Алгебра $C\otimes H$ интересна для меня и с другой точки зрения.
Поле комплексных чисел является алгебраическим замыканием поля действительных
чисел. Не возникает ли подобная связь между алгеброй $H$
и алгеброй $C\otimes H$?

В книге \citeBib{0812.4763},
на основе которой написана эта статья
я рассматриваю производные Гато функции тела.
Однако в этой статье я рассматриваю произвольные алгебры,
которые не всегда являются телом. В течении того времени,
что я работаю с производной Гато, я понял, что эта тема может быть
обобщена на более широкий класс алгебр.
Полное исследование появится позже, я написал эту статью с целью изучить
условия появления уравнения Коши\Hyph Римана.



==> Quaternion.Algebra.Russian.tex <==
%auto-ignore
\ifx\PrintBook\undefined
\else
\chapter{Алгебра кватернионов}
\label{chapter: Quaternion Algebra}
\fi

\input{\FilePrefix Complex.Number.Russian}

\input{\FilePrefix Quaternion.Algebra.Eq}

\section{Башня алгебр}
\label{section: Tower of Algebras}

Пусть $F_1$ - алгебра над полем $F_2$.
Пусть
\ShowEq{tower of algebras, basis 12}
- базис алгебры $F_1$ над полем $F_2$.
Пусть
\ShowEq{tower of algebras, structural constants 12}
- структурные константы
алгебры $F_1$ над полем $F_2$.

Пусть $F_2$ - алгебра над полем $F_3$.
Пусть
\ShowEq{tower of algebras, basis 23}
- базис алгебры $F_2$ над полем $F_3$.
Пусть
\ShowEq{tower of algebras, structural constants 23}
- структурные константы
алгебры $F_2$ над полем $F_3$.

%Доказать - башня представлений - $F_1$ - алгебра над полем $F_3$.

Я буду рассматривать алгебру $F_1$ как прямую сумму алгебр $F_2$.
Каждое слагаемое суммы я отождествляю с вектором базиса
\ShowEq{tower of algebras, basis 12}.
Соответственно, я могу рассматривать алгебру $F_1$ как алгебру над полем $F_3$.
Пусть $\Basis e_{13}$ - базис алгебры $F_1$ над полем $F_3$.
Индекс базиса
\ShowEq{tower of algebras, basis 13}
состоит из двух индексов: индекса слоя
и индекса вектора базиса
\ShowEq{tower of algebras, basis 23}
в слое.

Я буду отождествлять вектор базиса
\ShowEq{tower of algebras, e 12 i}
с единицей в соответствующем слое. Тогда
\ShowEq{Basis over F_2 and F_3}
Произведение векторов базиса $\Basis e_{13}$ имеет вид
\ShowEq{product of basis E13}
Так как $C_{12\cdot}{}_{\gi{ik}}^{\gi b}\in F_2$, то разложение
$C_{12\cdot}{}_{\gi{ik}}^{\gi b}$ относительно базиса
\ShowEq{tower of algebras, basis 23}
имеет вид
\ShowEq{structural constants 12 over 3}
Подставим \EqRef{structural constants 12 over 3}
в \EqRef{product of basis E13}
\ShowEq{product of basis E13, 1}
Следовательно, мы можем определить структурные константы
алгебры $F_1$ над полем $F_3$
\ShowEq{structural constants, F1 over F3}

Чтобы проверить построение, рассмотрим произведение
\ShowEq{structural constants, F1 over F3, 1}
С другой стороны
\ShowEq{structural constants, F1 over F3, 2}
Выражения \EqRef{structural constants, F1 over F3, 1},
\EqRef{structural constants, F1 over F3, 2} совпадают.

\begin{theorem}
\label{theorem: product F1 over F3, structural constants F1 in F3}
Если $C_{12\cdot}{}_{\gi{ik}}^{\gi b}\in F_3$, то компоненты
$\Vector e_{12\cdot\gi i}$,
$\Vector e_{23\cdot\gi k}$ вектора
$\Vector e_{13\cdot\gi{ik}}$ перемножаются независимо
\ShowEq{structural constants, F1 over F3, 3}
\end{theorem}
\begin{proof}
Из равенства \EqRef{product of basis E13} следует
\ShowEq{product of basis E13, 2}
Равенство \EqRef{structural constants, F1 over F3, 3}
следует из равенства \EqRef{product of basis E13, 2}.
\end{proof}

\begin{theorem}
\label{theorem: tower of algebra, coordinate structure}
Пусть $F_1$ - алгебра над полем $F_2$.
Пусть $F_2$ - алгебра над полем $F_3$.
Координаты
\ShowEq{a12}
элемента $a\in F_1$ относительно базиса
\ShowEq{tower of algebras, basis 12}
и координаты
\ShowEq{a13}
элемента $a\in F_1$ относительно базиса
\ShowEq{tower of algebras, basis 13}
связаны равенством
\ShowEq{a12a13}
\end{theorem}
\begin{proof}
Элемент $a\in F_1$ имеет разложение
\ShowEq{a12 1}
относительно базиса
\ShowEq{tower of algebras, basis 12}
и  разложение
\ShowEq{a13 1}
относительно базиса
\ShowEq{tower of algebras, basis 13}
Из равенств
\EqRef{Basis over F_2 and F_3},
\EqRef{a13 1},
следует
\ShowEq{a13 2}
Равенство
\EqRef{a12a13}
следует из равенств
\EqRef{a12 1},\EqRef{a13 2}.
\end{proof}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: tower of algebra, Cauchy Riemann equations}
Пусть $F_1$ - алгебра над полем $F_2$.
Пусть $F_2$ - алгебра над полем $F_3$.
Матрица $F_2$\Hyph линейного отображения
\ShowEq{f:F1->F1}
$F_2$\Hyph алгебры $F_1$
удовлетворяет соотношению
\ShowEq{tower of algebra, Cauchy Riemann equations}
\end{theorem}
\begin{proof}
Так как $f$ - $F_2$\Hyph линейное отображение, то
\ShowEq{tower of algebra, F_2 linear mapping}
Пусть
\ShowEq{tower of algebra, F_2 linear mapping, 1}
Тогда
\ShowEq{tower of algebra, F_2 linear mapping, 2}
Аналогично
\ShowEq{tower of algebra, F_2 linear mapping, 3}
Из равенств
\ShowEq{tower of algebra, F_2 linear mapping, 4}
следует
\ShowEq{tower of algebra, F_2 linear mapping, 5}
Так как
\ShowEq{tower of algebra, F_2 linear mapping, 6}
произвольны, то равенство
\EqRef{tower of algebra, Cauchy Riemann equations}
следует из равенства
\EqRef{tower of algebra, F_2 linear mapping, 5}
\end{proof}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: algebra, Cauchy Riemann equations}
Матрица $F_2$\Hyph линейного отображения
\ShowEq{f:F2->F2}
$F_3$\Hyph алгебры $F_2$
удовлетворяет соотношению
\ShowEq{algebra, Cauchy Riemann equations}
\end{theorem}
\begin{proof}
Утверждение теоремы будет доказано, если мы в теореме
\ref{theorem: tower of algebra, Cauchy Riemann equations}
положим $F_1=F_2$.
\end{proof}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: complex field, Cauchy Riemann equations}
Матрица $C$\Hyph линейного отображения
\ShowEq{f:C->C}
$R$\Hyph алгебры $C$
удовлетворяет соотношению
\ShowEq{complex field, Cauchy Riemann equations}
\end{theorem}
\begin{proof}
Для поля комплексных чисел $C$ уравнение
\EqRef{algebra, Cauchy Riemann equations}
имеет вид
\ShowEq{complex field, Cauchy Riemann equations, 1}
Из уравнений
\EqRef{structural constants of complex field},
\EqRef{complex field, Cauchy Riemann equations, 1},
следует
\ShowEq{complex field, Cauchy Riemann equations, 2}
Уравнения
\EqRef{complex field, Cauchy Riemann equations}
следует из уравнений
\EqRef{structural constants of complex field},
\EqRef{complex field, Cauchy Riemann equations, 2}.
\end{proof}

Я намеренно записал равенство
\EqRef{complex field, Cauchy Riemann equations, 2}
в промежуточной форме, чтобы показать насколько более
трудоёмко доказательство теоремы
\ref{theorem: complex field, Cauchy Riemann equations}
по сравнению с доказательством аналогичной теоремы
\ref{theorem: complex field over real field}.
Однако мы нигде не пользовались утверждением, что произведение
в $F_1$\Hyph алгебре $F_2$ коммутативно. Поэтому теорема
\ref{theorem: algebra, Cauchy Riemann equations}
может быть применена к произвольной алгебре.

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: quaternion, Cauchy Riemann equations}
Матрица $H$\Hyph линейного отображения
\ShowEq{f:H->H}
$R$\Hyph алгебры $H$
удовлетворяет соотношению
\ShowEq{quaternion, Cauchy Riemann equations}
\end{theorem}
\begin{proof}
Согласно теореме
\xRef{0812.4763}{theorem: Quaternion over real field}.
структурные константы алгебры кватернионов
имеют вид
\ShowEq{structural constants, quaternions E(R,-1,-1)}
Для алгебры кватернионов $H$ уравнение
\EqRef{algebra, Cauchy Riemann equations}
имеет вид
\ShowEq{quaternion, Cauchy Riemann equations, 1}
Из уравнений
\EqRef{structural constants, quaternions E(R,-1,-1)},
\EqRef{quaternion, Cauchy Riemann equations, 1},
следует\footnote{Я не рассматриваю равенства,
которые тривиальны или следуют из равенств
\EqRef{quaternion, Cauchy Riemann equations, 2}.}
\ShowEq{quaternion, Cauchy Riemann equations, 2}
Уравнения
\EqRef{quaternion, Cauchy Riemann equations}
следует из уравнений
\EqRef{structural constants, quaternions E(R,-1,-1)},
\EqRef{quaternion, Cauchy Riemann equations, 2}.
\end{proof}

\begin{theorem}
\label{theorem: tower of algebra, mapping structure}
Пусть $F_1$ - алгебра над полем $F_2$.
Пусть $F_2$ - алгебра над полем $F_3$.
Пусть $F_2$\Hyph линейное отображение
\ShowEq{f:F1->F1}
имеет представление
\ShowEq{f:F1->F1 12}
относительно базиса
\ShowEq{tower of algebras, basis 12}
и имеет представление
\ShowEq{f:F1->F1 13}
относительно базиса
\ShowEq{tower of algebras, basis 13}.
Координаты
\ShowEq{f13}
отображения $f$ относительно базиса
\ShowEq{tower of algebras, basis 13}
имеют вид
\ShowEq{f12f13}
\end{theorem}
\begin{proof}
Так как
\ShowEq{aj 23}
то, из равенства
\EqRef{f:F1->F1 12},
следует, что
\ShowEq{f:F1->F1 12 1}
Из равенства
\EqRef{f:F1->F1 13},
следует
\ShowEq{f:F1->F1 13 1}
Из равенств
\EqRef{f:F1->F1 12 1},
\EqRef{f:F1->F1 13 1},
следует
\ShowEq{f12f13 1}
Равенство
\EqRef{f12f13}
следует
из равенства
\EqRef{f12f13 1},
так как
\ShowEq{tower of algebras, basis 23}
- базис и координаты $a^{\gi{lj}}$ элемента $a\in F_1$
произвольны.
\end{proof}

\section{Алгебра кватернионов над полем комплексных чисел}

В этом разделе я буду рассматривать алгебру кватернионов $E(C,-1,-1)$,
где $C$ - поле комплексных чисел.

Произведение в алгебре $E(C,-1,-1)$ определено согласно таблице
\ShowEq{product of C quaternions over C}
Согласно теореме
\xRef{0812.4763}{theorem: Quaternion over real field}.
структурные константы алгебры кватернионов
имеют вид
\ShowEq{structural constants, quaternions E(C,-1,-1)}
Пусть $\Vector e_{23\cdot\gi k}=\Vector e_{C\cdot\gi k}$.
Произведение в алгебре $C$ определено согласно правилу
\EqRef{product of complex field}.
Согласно теореме
\ref{theorem: complex field over real field}
структурные константы поля комплексных чисел над полем действительных чисел
имеют вид
\EqRef{structural constants of complex field}

Следовательно, алгебра $E(C,-1,-1)$ изоморфна тензорному произведению
$C\otimes H$.
Поэтому можем выбрать базис
\ShowEq{product E(C,-1,-1) over real, basis}

\begin{theorem}
\label{theorem: product E(C,-1,-1) over real, table}
Таблица произведения алгебры $E(C,-1,-1)$ над полем $R$
имеет вид
\ShowEq{product E(C,-1,-1) over real, table}
\end{theorem}
\begin{proof}
Таблица записана согласно равенству
\ShowEq{product of basis  E(C,-1,-1) over real}
и определению базиса
\EqRef{product E(C,-1,-1) over real, basis}.
\end{proof}

\begin{theorem}
\label{theorem: structural constants, E(C,-1,-1) over real, table}
Структурные константы алгебры $E(C,-1,-1)$ над полем $R$ имеют вид
\ShowEq{structural constants, quaternions E(C,-1,-1) over real}
\end{theorem}
\begin{proof}
Утверждение теоремы можно рассматривать либо как следствие
теоремы \ref{theorem: product E(C,-1,-1) over real, table},
либо как следствие теоремы
\ref{theorem: product F1 over F3, structural constants F1 in F3}.
\end{proof}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: Quaternion E(C,-1,-1) over real field}
Матрица линейной функции
\ShowEq{Quaternion E(C,-1,-1) over real field, matrix of linear map}
алгебры $E(C,-1,-1)$
удовлетворяет соотношению
\ShowEq{Quaternion E(C,-1,-1) over real field, linear map}
\end{theorem}
\begin{proof}
Из равенств \xEqRef{0812.4763}{linear map over field, division ring, relation},
\EqRef{structural constants, F1 over F3, 3},
\EqRef{structural constants of complex field}
следует
\ShowEq{Quaternion E(C,-1,-1) over real field, linear map, 1}
Равенство \EqRef{Quaternion E(C,-1,-1) over real field, linear map}
следует из сравнения равенств
\eqref{Quaternion E(C,-1,-1) over real field, linear map, 1, 1}
и
\eqref{Quaternion E(C,-1,-1) over real field, linear map, 1, 4},
\eqref{Quaternion E(C,-1,-1) over real field, linear map, 1, 2}
и
\eqref{Quaternion E(C,-1,-1) over real field, linear map, 1, 3}.
\end{proof}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: Quaternion E(C,-1,-1) over real field, jacobian}
Если матрица
\ShowEq{Quaternion E(C,-1,-1) over real field, jacobian, 1}
является матрицей Якоби функции в алгебре $E(C,-1,-1)$,
то
\ShowEq{Quaternion E(C,-1,-1) over real field, jacobian, 2}
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: Quaternion E(C,-1,-1) over real field}.
\end{proof}

\section{Алгебра \texorpdfstring{\ShowEq{algebra CCH}}{Cx(CxH)}}

Алгебра \ShowEq{algebra CCH} не является алгеброй кватернионов.
Однако я рассматриваю здесь эту алгебру так как в некотором смысле
эта алгебра похожа на алгебру $E(C,-1,-1)=C\otimes H$.

Алгебра \ShowEq{algebra CCH}
интересна и с другой точки зрения.
При рассмотрении этой алгебры становится очевидным,
что тензорное произведение некоммутативных колец неассоциативно.
Так как $C$ - поле, то $C\otimes C$ изоморфно $C$, и следовательно,
$(C\otimes C)\otimes H$ изоморфно $C\otimes H$.
Однако, так как $H$ не является алгеброй над полем комплексных чисел,
то алгебра
\ShowEq{algebra CCH}
отличается от алгебры
$(C\otimes C)\otimes H=C\otimes H$.

Алгебра \ShowEq{algebra CCH} имеет настолько большую размерность,
что становится нецелесообразным рассматривать таблицу умножения
и структурные константы этой алгебры.
Однако нетрудно увидеть, что структура этой алгебры
во многом похожа на структуру алгебр, рассмотренных в разделе
\ref{section: Tower of Algebras}.

Мы будем представлять базис алгебры \ShowEq{algebra CCH}
в виде
\ShowEq{algebra CCH, basis}
где $\Basis e_C$ - базис алгебры $C$
и $\Basis e_H$ - базис алгебры $H$.
Соответственно, произведение в алгебре
\ShowEq{algebra CCH} определено покомпонентно
\ShowEq{algebra CCH, product}

\begin{theorem}
\label{theorem: structural constants, algebra CCH}
Структурные константы алгебры \ShowEq{algebra CCH} имеют вид
\ShowEq{structural constants, algebra CCH}
где $C_{C\cdot}{}_{\gi{pq}}^{\gi r}$ - структурные константы поля
комплексных чисел, $C_{H\cdot}{}_{\gi{ik}}^{\gi b}$ - структурные
константы алгебры кватернионов.
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно сравнить
следующие равенства
\ShowEq{structural constants, algebra CCH, proof}
\end{proof}

\begin{theorem}
\label{theorem: structural constants, algebra CCH, table}
Структурные константы алгебры \ShowEq{algebra CCH} имеют вид
\ShowEq{structural constants, algebra CCH, table}
\end{theorem}
\begin{proof}
Утверждение теоремы является следствием
теорем \ref{theorem: structural constants, algebra CCH},
\ref{theorem: complex field over real field}.
\end{proof}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: algebra CCH, Cauchy Riemann equation}
Матрица линейной функции
\ShowEq{algebra CCH, matrix of linear map}
алгебры \ShowEq{algebra CCH}
удовлетворяет соотношению
\ShowEq{algebra CCH, Cauchy Riemann equation}
\end{theorem}
\begin{proof}
Опираясь на равенства
\xEqRef{0812.4763}{linear map over field, division ring, relation},
\EqRef{structural constants, algebra CCH, table},
мы можем повторить вычисления, выполненные для доказательства теоремы
\ref{theorem: Quaternion E(C,-1,-1) over real field}.
Однако очевидно, что эти вычисления отличаются только набором
индексов. Таким образом, из теоремы
\ref{theorem: Quaternion E(C,-1,-1) over real field}
следует
\ShowEq{algebra CCH, Cauchy Riemann equation, proof}
Равенства \EqRef{algebra CCH, Cauchy Riemann equation, linear map}
следуют из равенств
\EqRef{algebra CCH, Cauchy Riemann equation, proof, 1},
\EqRef{algebra CCH, Cauchy Riemann equation, proof, 2}.
\end{proof}

\begin{theorem}[Уравнения Коши\Hyph Римана]
\label{theorem: algebra CCH, Cauchy Riemann equation, jacobian}
Если матрица
\ShowEq{algebra CCH, Cauchy Riemann equation, jacobian, 1}
является матрицей Якоби функции в алгебре \ShowEq{algebra CCH},
то
\ShowEq{algebra CCH, Cauchy Riemann equation, jacobian, 2}
\end{theorem}
\begin{proof}
Следствие теоремы
\ref{theorem: algebra CCH, Cauchy Riemann equation}.
\end{proof}

\section{Алгебра кватернионов \texorpdfstring{$E(R,a,b)$}{E(R,a,b)}}

Положим $\Vector e_{\gi 0}=1$, $\Vector e_{\gi 1}=i$,
$\Vector e_{\gi 2}=j$, $\Vector e_{\gi 3}=k$.
Согласно равенству
\EqRef{product in E(F,a,b), table}
структурные константы алгебры $E(R,a,b)$ имеют вид
\ShowEq{structural constants of algebra E(R,a,b)}

\begin{theorem}
\label{theorem: Quaternion E(R,a,b)}
Стандартные компоненты линейной функции
и координаты соответствующего линейного преобразования над полем $R$
удовлетворяют соотношениям
\ShowEq{Quaternion E(R,a,b)}
\end{theorem}
\begin{proof}
Пользуясь равенством
\xRef{0812.4763}{eq: linear map over field, division ring, relation}
получаем соотношения
\ShowEq{Quaternion E(R,a,b), 1}
Мы группируем эти соотношения в системы линейных уравнений
\EqRef{Quaternion E(R,a,b), 1, 0},
\EqRef{Quaternion E(R,a,b), 1, 1},
\EqRef{Quaternion E(R,a,b), 1, 2},
\EqRef{Quaternion E(R,a,b), 1, 3}.

\EqRef{Quaternion E(R,a,b), 2, 0} -
это решение системы линейных уравнений
\EqRef{Quaternion E(R,a,b), 1, 0}.

\EqRef{Quaternion E(R,a,b), 2, 1} -
это решение системы линейных уравнений
\EqRef{Quaternion E(R,a,b), 1, 1}.

\EqRef{Quaternion E(R,a,b), 2, 2} -
это решение системы линейных уравнений
\EqRef{Quaternion E(R,a,b), 1, 2}.

\EqRef{Quaternion E(R,a,b), 2, 3} -
это решение системы линейных уравнений
\EqRef{Quaternion E(R,a,b), 1, 3}.
\end{proof}

\begin{theorem}
Для любых значений параметров $a\ne 0$, $b\ne 0$,
существует взаимно однозначное соответствие между координатами
линейной функции алгебры $E(R,a,b)$ и её стандартными компонентами.
\end{theorem}
\begin{proof}
Следствие теоремы \ref{theorem: Quaternion E(R,a,b)}.
\end{proof}

\section{Регулярная функция}

Хотя в алгебре кватернионов нет аналога уравнения Коши\Hyph Римана,
в различных статьях изучаются различные множества функций, свойства которых
похожи на свойства функций комплексного переменного.
В \citeBib{Fueter,Sudbery Quaternionic Analysis}
определена регулярная функция, которая удовлетворяет
уравнению
\ShowEq{Regular quaternion function, 1}

\begin{theorem}
\label{theorem: Regular quaternion function, differential equation}
Дифференциальное уравнение
\EqRef{Regular quaternion function, 1}
эквивалентно системе дифференциальных уравнений
\ShowEq{Regular quaternion function, differential equation}
\end{theorem}
\begin{proof}
Подставив
\ShowEq{Regular quaternion function, 3, 0}
в уравнение
\EqRef{Regular quaternion function, 1}, получим
\ShowEq{Regular quaternion function, 4}
Утверждение теоремы следует из равенства
\EqRef{Regular quaternion function, 4}.
\end{proof}

В статье \citeBib{C.A. Deavours The Quaternion Calculus},
следствие 3.1.2, p. 1000,
показано, что если регулярная функция над алгеброй кватернионов
имеет ограниченную норму, то это функция
тождественно постоянна.

\begin{theorem}
\label{theorem: Regular quaternion function, Gateaux derivative, components}
Компоненты производной Гато регулярной функции
над алгеброй кватернионов удовлетворяют равенствам
\ShowEq{Regular quaternion function, Gateaux derivative, components}
\end{theorem}
\begin{proof}
Подставив уравнения
\ShowEq{quaternion over real field, derivative}
в уравнения \EqRef{Regular quaternion function, differential equation},
мы получим
\ShowEq{Regular quaternion function, 6, 0}
\end{proof}

\begin{theorem}
Дифференциал Гато регулярной функции над алгеброй кватернионов имеет вид
\ShowEq{Regular quaternion function, Gateaux differential}
\end{theorem}
\begin{proof}
Утверждение теоремы является
следствием теоремы
\xRef{0812.4763}
{theorem: Gateaux differential, standard form, division ring}.
\end{proof}

Равенство \EqRef{Regular quaternion function, 1}
эквивалентно равенству
\ShowEq{Regular quaternion function, 3}
\ifx\texFuture\Defined
Производная Гато функции над алгеброй кватернионов является
полным дифференциалом и имеет вид
\ShowEq{Gateaux derivative, quaternion function}
где
\ShowEq{Gateaux derivative, quaternion function, 1}
Поэтому символическое уравнение
\ShowEq{Cauchy Riemann equations, Gateaux derivative, Regular quaternion function}
не выражает связь производной Гато с уравнения Коши\Hyph Римана.

\section{Slice Regular Function}

Согласно определению \citeBib{0902.4771}-1.1,
функция, удовлетворяющая уравнению
\ShowEq{Slice Regular Function}
для любого кватерниона $I=I_{\gi 1}i+I_{\gi 2}j+I_{\gi 3}k$ такого, что
$I_{\gi 1}^2+I_{\gi 2}^2+I_{\gi 3}^2=1$.
называется slice regular function.

Мы здесь рассматриваем производную составной функции
и согласно теореме
\xRef{0812.4763}{theorem: composite map, differential, D vector space}
эту производную можно представить в виде
\ShowEq{Slice Regular Function, 01}

------

\begin{theorem}
\label{theorem: Slice Regular quaternion function, differential equation}
Дифференциальное уравнение
\EqRef{Slice Regular Function}
эквивалентно системе дифференциальных уравнений
\ShowEq{Slice Regular quaternion function, differential equation}
\end{theorem}
\begin{proof}
Так как
\ShowEq{Slice Regular quaternion function, 3, 0}
то уравнение
\EqRef{Slice Regular Function}
можно записать с помощью матриц
\ShowEq{Slice Regular quaternion function, 3}
Подставив \EqRef{Slice Regular quaternion function, 3, 0} в уравнение
\EqRef{Slice Regular Function}, получим
\ShowEq{Slice Regular quaternion function, 4}
Утверждение теоремы следует из равенства
\EqRef{Slice Regular quaternion function, 4}.
\end{proof}

Я не буду продолжать рассчёт дальше. Очевидно, что также
как и для регулярных функций, мы можем выписать общую форму
дифференциала. При этом надо учитывать возможность
равенства $0$ величин $a_{\gi i}$.

\section{}
Пусть
\[
f:D\rightarrow D
\]
непрерывное отображение. Пусть $\Basis e$ - базис тела $D$ над
центром $Z(D)$.
Производная Гато отображения $f$ в базисе $\Basis e$ имеет вид
\ShowEq{Gateaux derivative map f basis e, quaternion}
Для вектора $\Vector e_{\gi k}$ справедливо равенство
\ShowEq{Gateaux derivative map f basis e, 1, quaternion}
Из равенств
\EqRef{Gateaux derivative map f basis e, quaternion},
\EqRef{Gateaux derivative map f basis e, 1, quaternion}
следует
\ShowEq{Gateaux derivative map f basis e, 2, quaternion}
Если отображение $f$ невырождено, то векторы
\EqRef{Gateaux derivative map f basis e, 2, quaternion}
также порождают локальный базис
\ShowEq{Gateaux derivative map f basis e, 3, quaternion}
определённый в каждой точке тела $D$.
Согласно \citeBib{Cartan geometry in reper},
с. 8,
мы можем рассматривать множество векторов
$\Vector e'_{\gi k}(x)$
как подвижной репер. Соответствующие уравнения имеют вид
\ShowEq{moving frame, division ring}
Мы будем полагать, что в локальном базисе определено скалярное
произведение
\ShowEq{scalar product in local basis, quaternion algebra}

Предположим, что отображение $f$ конформно,
т. е. производная этого отображения сохраняет углы.
Если исходный базис ортогонален, то базис $\Basis e'(x)$
также ортогонален
\ShowEq{scalar product in local basis 1, quaternion algebra}

Связность в новых координатах имеет вид
\[
\Gamma'^p_{ji}
=\frac{\partial x'^p}{\partial x^r}
\frac{\partial^2 x^r}{\partial x'^j\partial x'^i}
\]
Кривизна имеет вид
\[
R_{lki}^q=\frac{\partial \Gamma^q_{li}}{\partial x^k}
-\frac{\partial \Gamma^q_{ki}}{\partial x^l}
+\Gamma^q_{kp}\Gamma^p_{li}
-\Gamma^q_{lp}\Gamma^p_{ki}
\]
\begin{align*}
R_{lki}^q&=\frac{\frac{\partial x'^q}{\partial x^r}
\frac{\partial^2 x^r}{\partial x'^l\partial x'^i}}{\partial x^k}
-\frac{\frac{\partial x'^q}{\partial x^r}
\frac{\partial^2 x^r}{\partial x'^k\partial x'^i}}{\partial x^l}
\\
&+\frac{\partial x'^q}{\partial x^r}
\frac{\partial^2 x^r}{\partial x'^k\partial x'^p}
\frac{\partial x'^p}{\partial x^s}
\frac{\partial^2 x^s}{\partial x'^l\partial x'^i}
-\frac{\partial x'^q}{\partial x^r}
\frac{\partial^2 x^r}{\partial x'^l\partial x'^p}
\frac{\partial x'^p}{\partial x^s}
\frac{\partial^2 x^s}{\partial x'^k\partial x'^i}
\end{align*}

Мы будем полагать, что в алгебре кватернионов определено скалярное
произведение
\ShowEq{scalar product, quaternion algebra}
\fi

